From Similarity to Superiority: Channel Clustering for Time Series Forecasting

Time series forecasting has attracted significant attention in recent decades. Previous studies have demonstrated that the Channel-Independent (CI) strategy improves forecasting performance by treating different channels individually, while it leads to poor generalization on unseen instances and ignores potentially necessary interactions between channels. Conversely, the Channel-Dependent (CD) strategy mixes all channels with even irrelevant and indiscriminate information, which, however, results in oversmoothing issues and limits forecasting accuracy. There is a lack of channel strategy that effectively balances individual channel treatment for improved forecasting performance without overlooking essential interactions between channels. Motivated by our observation of a correlation between the time series model's performance boost against channel mixing and the intrinsic similarity on a pair of channels, we developed a novel and adaptable Channel Clustering Module (CCM). CCM dynamically groups channels characterized by intrinsic similarities and leverages cluster information instead of individual channel identities, combining the best of CD and CI worlds. Extensive experiments on real-world datasets demonstrate that CCM can (1) boost the performance of CI and CD models by an average margin of 2.4% and 7.2% on long-term and short-term forecasting, respectively; (2) enable zero-shot forecasting with mainstream time series forecasting models; (3) uncover intrinsic time series patterns among channels and improve interpretability of complex time series models.

==> chapters/checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Clearly state the contribution in the introduction.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Discussed the limitations in conclusion.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper does not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Provided implementation and hyperparameters in Appendix~\ref{appd:exp_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code is available at \url{https://github.com/Graph-and-Geometric-Learning/TimeSeriesCCM}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Provide training and test details in Appendix~\ref{appd:exp_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Provided error bars in Appendix~\ref{appd:exp_error}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Provided details in Appendix~\ref{appd:exp_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: well conform with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Discussed the social impacts in Appendix~\ref{app:discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: the paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Cited the original paper that produced the dataset used in this work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Will document the newly released dataset and well specify the license after paper acceptance.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/abstract.tex <==
\begin{abstract}
    Large language models (LLMs) have demonstrated impressive reasoning abilities in complex tasks. However, they lack up-to-date knowledge and experience hallucinations during reasoning, which can lead to incorrect reasoning processes and diminish their performance and trustworthiness. Knowledge graphs (KGs), which capture vast amounts of facts in a structured format, offer a reliable source of knowledge for reasoning. Nevertheless, existing KG-based LLM reasoning methods only treat KGs as factual knowledge bases and overlook the importance of their structural information for reasoning. 
    %
    In this paper, we propose a novel method called reasoning on graphs (\ourmethod) that synergizes LLMs with KGs to enable faithful and interpretable reasoning. Specifically, we present a planning-retrieval-reasoning framework, where \ourmethod first generates relation paths grounded by KGs as faithful plans. These plans are then used to retrieve valid reasoning paths from the KGs for LLMs to conduct faithful reasoning. Furthermore, \ourmethod not only distills knowledge from KGs to improve the reasoning ability of LLMs through training but also allows seamless integration with any arbitrary LLMs during inference. Extensive experiments on two benchmark KGQA datasets demonstrate that \ourmethod achieves state-of-the-art performance on KG reasoning tasks and generates faithful and interpretable reasoning results\footnote{Code and data are available at: \url{https://github.com/RManLuo/reasoning-on-graphs}}.
\end{abstract}

==> sections/acknowledgement.tex <==
\section*{Acknowledgments}
This material is based on research partially sponsored by the DARPA Assured Neuro Symbolic Learning and Reasoning (ANSR) program under award number FA8750-23-2-1016 and the DARPA Knowledge Management at Scale and Speed (KMASS) program under award number HR00112220047. This research is partly supported by the ARC Future Fellowship FT190100039 to G.H. S. Pan was supported in part by the Australian Research Council (ARC) under grants FT210100097 and DP240101547, and the CSIRO – National Science Foundation (US) AI Research Collaboration Program.

==> sections/approach.tex <==
\begin{figure}[]
    \begin{center}
    %\framebox[4.0in]{$\;$}
    \includegraphics[width=.85\columnwidth]{images/RoG.pdf}
    \end{center}
    \vspace{-3mm}
    \caption{The overall framework of reasoning on graphs (\ourmethod). \RE{1) given a question, we first prompt LLMs to generate several relation paths that are grounded by KGs as plans. 2) Then, we retrieve reasoning paths from KGs using the plans. 3) Finally, we conduct faithful reasoning based on the retrieved reasoning paths and generate answers with interpretable explanations. The orange and red rectangles denote the entities mentioned in the question and answer, respectively.}}
    \label{fig:framework}
    \vspace{-5mm}
\end{figure}

\section{Approach}
% In this section, we introduce our method: reasoning on graphs (\ourmethod). We present a novel \textit{planning-retrieval-reasoning} framework that synergizes LLMs and KGs to conduct faithful and interpretable reasoning for KGQA. The overall framework of \ourmethod is illustrated in \Cref{fig:framework}.


\RE{In this section, we introduce our method: reasoning on graphs (\ourmethod), which contains two components: 1) a \textit{planning} module that generates relation paths grounded by KGs as faithful plans; 2) a \textit{retrieval-reasoning} module that first retrieves valid reasoning paths from KGs according to the plans, then conducts faithful reasoning based on retrieved reasoning paths and generates answers with interpretable explanations. The overall framework of \ourmethod is illustrated in \Cref{fig:framework}.}


\subsection{Reasoning on Graphs: Planning-Retrieval-Reasoning}

Recently, many techniques have been explored to improve the reasoning ability of LLMs by planning, which first prompts LLMs to generate a reasoning plan and then conduct reasoning based on it \citep{wang2023plan}. However, LLMs are known for having hallucination issues, which are prone to generating incorrect plans and leading to wrong answers \citep{ji2023survey}.
%
To address this issue, we present a novel \textit{planning-retrieval-reasoning} framework, which makes the reasoning plans grounded by KGs and then retrieves faithful reasoning paths for LLM reasoning. 

Relation paths, which capture semantic relations between entities, have been utilized in many reasoning tasks on KGs \citep{wang2021relational,xusubgraph}. Moreover, compared to the dynamically updated entities, the relations in KGs are more stable \citep{wang2023survey}. By using relation paths, we can always retrieve the latest knowledge from KGs for reasoning. Therefore, relation paths can serve as faithful plans for reasoning the answer to KGQA task.
\begin{example}
    Given a question ``Who is the child of Alice'', we can generate a relation path as the plan: $z=\texttt{marry\_to} \to \texttt{father\_of}$. This relation path expresses the plan: 1) find the person that ``Alice'' is married to; 2) find the child of that person.
    We can execute the plan (relation path) by retrieving a reasoning path from KGs as: $w_z=\text{Alice}\xrightarrow{\texttt{marry\_to}}\text{Bob}\xrightarrow{\texttt{father\_of}}\text{Charlie}$. Finally, we can answer the question based on the reasoning path, which is ``Charlie''.
\end{example}

By treating relation paths as plans, we can make sure the plans are grounded by KGs, which enables LLMs to conduct faithful and interpretable reasoning on graphs. In a nutshell, we formulate our \ourmethod as an optimization problem that aims to maximize the probability of reasoning the answer from a knowledge graph $\gG$ w.r.t the question $q$ by generating relation paths $z$ as the plan:
% Thus, the objective function of our \ourmethod can be formulated as
\begin{equation}
    \setlength\abovedisplayskip{1pt}%shrink space
    \setlength\belowdisplayskip{1pt}
    \label{eq:plan}
    P_\theta(a|q,\gG) = \sum_{z\in\gZ}P_\theta(a|q,z,\gG)P_\theta(z|q),
\end{equation}
where $\theta$ denotes the parameters of LLMs, $z$ denotes the relation paths (plans) generated by LLMs, and $\gZ$ denotes the set of possible relation paths. The latter term $P_\theta(z|q)$ is the probability of generating a faithful relation path $z$ grounded by KG, given the question $q$, which is realized by the \textit{planning} module. The former term $P_\theta(a|q,z,\gG)$ is the probability of reasoning an answer $a$ given the question $q$, relation path $z$, and KG $\gG$, which is computed by the \textit{retrieval-reasoning} module.

\subsection{Optimization Framework}
Despite the advantage of generating relation paths as plans, the LLMs have zero knowledge of the relations contained in KGs. Therefore, LLMs cannot directly generate relation paths grounded by KGs as faithful plans. Moreover, LLMs might not understand the reasoning paths correctly and conduct reasoning based on them. To address these issues, we design two instruction tuning tasks: 1) \textit{planning optimization}, which distills the knowledge from KGs into LLMs to generate faithful relation paths as plans; 2) \textit{retrieval-reasoning optimization}, which enables LLMs to reason based on the retrieved reasoning paths.

The objective function in \eqref{eq:plan} can be optimized by maximizing the evidence lower bound (ELBO) \citep{jordan1999introduction}, which is formulated as
\begin{equation}
    \log P(a|q,\gG) \geq \E_{z\sim Q(z)}[\log P_\theta(a|q,z,\gG)] - \KL(Q(z)\Vert P_\theta(z|q)),
\end{equation}
where $Q(z)$ denotes the posterior distribution of faithful relation paths grounded by KGs. The latter term minimizes the KL divergence between the posterior and the prior, which encourages LLMs to generate faithful relation paths (planning optimization). The former term maximizes the expectation that retrieval-reasoning module generates correct answers based on the relation paths and KGs (retrieval-reasoning optimization). 

\noindent\textbf{Planning optimization.} In planning optimization, we aim to distill the knowledge from KGs into LLMs to generate faithful relation paths as plans. This can be achieved by minimizing the KL divergence with the posterior distribution of faithful relation paths $Q(z)$, which can be approximated by the valid relation paths in KGs. 

Given a question $q$ and answer $a$, we could find the path instances $w_z(e_q,e_a)=e_q\xrightarrow{r_1}e_1\xrightarrow{r_2}\ldots\xrightarrow{r_l}e_{a}$ connecting $e_q$ and $e_a$ in KGs. The corresponding relation path $z=\{r_1,r_2,\dots,r_l\}$ can be considered valid and serve as a faithful plan for answering the question $q$. The posterior distribution $Q(z)$ can be formally approximated as
\begin{equation}
    \setlength\abovedisplayskip{1pt}%shrink space
    \setlength\belowdisplayskip{1pt}
    \label{eq:posterior}
    Q(z) \simeq Q(z|a, q, \gG)=
    \left\{
    \begin{aligned}
         & \RE{\frac{1}{|\mathcal{Z}|}}, \exists w_z(e_q,e_a) \in \gG, \\
         & 0, else,
    \end{aligned}
    \right.
\end{equation}
where \RE{ we assume a uniform distribution over all valid relation paths $\mathcal{Z}$}, and $\exists w_z(e_q,e_a) \in \gG$ denote the existence of a path instance connecting the question $e_q$ and answer $e_a$ entities in $\gG$.
%
Therefore, the KL divergence can be calculated as
\begin{equation}
    \setlength\abovedisplayskip{1pt}%shrink space
    \setlength\belowdisplayskip{1pt}
    \label{eq:kl}
    \gL_{\text{plan}}=\KL(Q(z)\Vert P_\theta(z|q)) = \KL(Q(z|a, q, \gG)\Vert P_\theta(z|q)) \RE{~\simeq - \frac{1}{|\gZ^*|}\sum_{z\in\gZ^*} \log P_\theta(z|q),}
\end{equation}
\RE{where we use the shortest paths $\gZ^*\subseteq\mathcal{Z}$ between $e_q$ and $e_a$ in KGs as supervision signals \citep{zhang2022subgraph}.} The detailed derivation of can be found in \Cref{app:planning_derivation}.
By optimizing the \eqref{eq:kl}, we maximize the probability of LLMs generating faithful relation paths through distilling the knowledge from KGs.

\noindent\textbf{Retrieval-reasoning optimization.} In retrieval-reasoning optimization, we aim to enable LLMs to conduct reasoning based on the retrieved reasoning paths. 
For the retrieval-reasoning module, we follow the FiD framework \citep{izacard2021leveraging,singh2021end}, which allows reasoning on multiple retrieved reasoning paths\footnote{\RE{The FiD framework assumes each $z\in \mathcal{Z}$ contributes independently, where the probability $P_\theta(a|q,\mathcal{Z},\mathcal{G})$ can be approximated as the product of each $P_\theta(a|q,z,\gG)$.}}, formulated as
\begin{equation}
    \setlength\abovedisplayskip{1pt}%shrink space
    \setlength\belowdisplayskip{1pt}
    P_\theta(a|q,\gZ,\gG) = \prod_{z\in\gZ}P_\theta(a|q,z,\gG).
\end{equation}

By approximating the expectation with \RE{K sampled plans $\gZ^{*}_{K}\subseteq Z^*$}, the objective function of reasoning optimization can be written as
\begin{equation}
    \setlength\abovedisplayskip{1pt}%shrink space
    \setlength\belowdisplayskip{1pt}
    \gL_{\text{reason}}= \E_{z\sim Q(z|a, q, \gG)}[\log P_\theta(a|q,z,\gG)] \RE{ = \sum_{z\in\gZ^*_K} \log P_\theta(a|q,z,\gG)} =  \log P_\theta(a|q,\gZ^*_{K},\gG).
\end{equation}
This maximizes the probability of LLMs generating correct answers based on the retrieved reasoning paths.

The final objective function of \ourmethod is the combination of the planning optimization and retrieval-reasoning optimization, which can be formulated as
\begin{equation}
    \setlength\abovedisplayskip{1pt}%shrink space
    \setlength\belowdisplayskip{1pt}
    \label{eq:final_obj}
    \gL = \log \underbrace{P_\theta(a|q,\RE{\gZ^*_K},\gG)}_{\text{Retrieval-reasoning}} + \underbrace{\RE{\frac{1}{|\gZ^*|}}\sum_{z\in \RE{Z^*}}\log P_\theta(z|q)}_{\text{Planning}}.
\end{equation}
From \eqref{eq:final_obj}, we can see that we adopt the same LLM for both planning and reasoning, which are jointly trained on two instruction-tuning tasks, i.e., (planning and retrieval-reasoning). We will discuss the implementation details of these two tasks in the following subsections.

\subsection{Planning Module}
The planning module aims to generate faithful relation paths as plans for answering the question. To utilize the instruction-following ability of LLMs \citep{wei2021finetuned}, we design a simple instruction template that prompts LLMs to generate relation paths:

% \LH{Any better way to present the instruction template?}
\begin{minipage}{0.99\columnwidth}
    \centering
    \begin{tcolorbox}
        \small
        Please generate a valid relation path that can be helpful for answering the following question: \texttt{<Question>}
    \end{tcolorbox}
    \vspace{1mm}
\end{minipage}
where \texttt{<Question>} indicates the question $q$. The question together with the instruction template is fed into LLMs to generate the relation paths, which are structurally formatted as a sentence:

\begin{minipage}{0.99\columnwidth}
    \centering
    $z=$ \texttt{<PATH>} $r_1$ \texttt{<SEP>}  $r_2$ \texttt{<SEP>} $\dots$ \texttt{<SEP>} $r_l$ \texttt{</PATH>}
    \vspace{1mm}
\end{minipage}
where \texttt{<PATH>}, \texttt{<SEP>}, \texttt{</PATH>} are special tokens indicating the start, separator, and end of the relation path, respectively\footnote{The relation name $r_*$ could be split into multiple tokens. For example, ``\texttt{born\_in}'' could be split into ``\texttt{born}'' and ``\texttt{\_in}'' by tokenizer. In this way,  we could fully utilize the semantic information in relation names and generalize to different KGs.}. 

Therefore, the optimization of $\gL_{\text{plan}}$ can be achieved as
\begin{equation}
    \setlength\abovedisplayskip{1pt}%shrink space
    \setlength\belowdisplayskip{1pt}
    \argmax_\theta \RE{\frac{1}{|\gZ^*|}}\sum_{z\in \RE{\gZ^*}} \log P_\theta(z|q)= \RE{\frac{1}{|\gZ^*|}} \sum_{z\in \RE{\gZ^*}}\log \prod_{i=1}^{|z|}P_\theta(r_i|r_{<i},q),
\end{equation}
where $P_\theta(z|q)$ denotes the prior distribution of generating faithful relation path $z$, and $P_\theta(r_i|r_{<i},q)$ denotes the probability of each token in $z$ generated by LLMs.

\subsection{Retrieval-Reasoning Module}

\noindent\textbf{Retrieval}. Given a question $q$ and a relation path as plan $z$, the retrieval module aims to retrieve the reasoning paths $w_z$ from KG $\gG$. The retrieval process can be conducted by finding paths in $\gG$ that start from the question entities $e_q$ and follow the relation paths $z$, formulated as
\begin{equation}
    \setlength\abovedisplayskip{1pt}%shrink space
    \setlength\belowdisplayskip{1pt}
    \gW_z=\{w_z(e_q,e_*)|w_z(e_q,e_*)=e_q\xrightarrow{r_1}e_1\xrightarrow{r_2}\ldots\xrightarrow{r_l}e_{a*}, w_z(e_q,e_*)\in\gG\}.
\end{equation}
We adopt a constrained breadth-first search to retrieve the reasoning paths $w_z$ from KGs. In experiments, all retrieved paths are used for reasoning. The detailed retrieval algorithm can be found in \Cref{app:retrieval}.

Despite we can utilize the retrieved reasoning paths and directly get the answers with majority voting. The retrieved reasoning paths could be noisy and irrelevant to the questions, which leads to incorrect answers \citep{he2021improving,zhang2022subgraph}. Therefore, we propose a reasoning module to explore the ability of LLMs to identify the important reasoning paths and answer the questions based on them.
% The probability of retrieving the reasoning path $w_z$ from KGs given the relation path $z$ is formulated as
% \begin{equation}
%     \label{eq:posterior}
%     P(w_z|z,q,\gG)
%     \left\{
%     \begin{aligned}
%          & 1, \exists w_z(e_q,e_*) \in \gG, \\
%          & 0, else.
%     \end{aligned}
%     \right.
% \end{equation}

\noindent\textbf{Reasoning}. The reasoning module takes the question $q$ and a set of reasoning paths $\gW_z$ to generate answers $a$. 
Similarly, we design a reasoning instruction prompt to guide LLMs to conduct reasoning based on the retrieved reasoning paths $\gW_z$. The $\gW_z$ are also formatted as a series of structural sentences.
%
% where \texttt{<Reasoning Paths>} denotes the retrieved reasoning paths $\gW_z$ which are formatted as a series of structural sentences.
%
% \begin{minipage}{0.99\columnwidth}
%     \centering
%     $x_z=e_1 \to r_1 \to e_2 \to \dots \to r_l \to e_l,w_z\in\gW_z$.
%     \vspace{1mm}
% \end{minipage}
The detailed prompt can be found in \Cref{app:prompts}. 

The optimization of $\gL_{\text{reason}}$ can be written as
\begin{equation}
    \setlength\abovedisplayskip{1pt}%shrink space
    \setlength\belowdisplayskip{1pt}
    \argmax_\theta \log P_\theta(a|q,\RE{\gZ^*_K},\gG) =  \log \sum_{z\in\RE{\gZ^*_K}}\sum_{w_z\in\gW_z}\prod_{i=1}^{|a|}P_\theta(t_i|t_{<i},q,w_z),
\end{equation}
where $P_\theta(a|q,\gZ_K,\gG)$ denotes probability of reasoning the correct answer $a$ based on $K$ relation paths $\gZ_K$, and $t_*$ denote the tokens of answers $a$.

% \subsection{Optimization}

% The \eqref{eq:plan} can be optimized by maximizing the evidence lower bound (ELBO) \citep{jordan1999introduction}, which can be formulated as
% \begin{equation}
%     \log P(a|q,\gG) \geq \E_{z\sim Q(z)}[\log P_\theta(a|q,z,\gG)] - \KL(Q(z)\Vert P_\theta(z|q)),
% \end{equation}
% where $Q(z)$ denotes the posterior distribution of faithful reasoning plans grounded by KGs. The first term maximizes the expectation that retrieval-then-reasoning module generates correct answers based on the plans. The second term minimizes the KL divergence between the posterior and the prior, which distills the knowledge from KGs and encourages LLM to generate faithful reasoning plans.

% The posterior distribution of faithful plans $Q(z)$ can be approximated by valid relation paths on KGs. Given a question $q$ and answer $a$, we found the shortest paths $w_z(e_q,e_a)=e_q\xrightarrow{r_1}e_1\xrightarrow{r_2}\ldots\xrightarrow{r_l}e_{a}$ connecting $e_q$ and $e_a$ in KGs. Therefore, the valid relation path $z=\{r_1,r_2,\dots,r_l\}$ can be served as a faithful plan for answering the question $q$ and the posterior distribution $Q(z)$ can be formally approximated as
% \begin{equation}
%     \label{eq:posterior}
%     Q(z) \simeq Q(z|a, q, \gG)=
%     \left\{
%     \begin{aligned}
%          & 1, \exists w_z(e_q,e_a) \in \gG, \\
%          & 0, else.
%     \end{aligned}
%     \right.
% \end{equation}

% Therefore, the KL divergence can be calculated as
% \begin{equation}
%     \begin{aligned}
%         \KL(Q(z)\Vert P_\theta(z|q)) &= \KL(Q(z|a, q, \gG)\Vert P_\theta(z|q)) \\
%         &= \E_{z\sim Q(z|a, q, \gG)}Q(z|a, q, \gG)[\log Q(z|a, q, \gG)-\log P_\theta(z|q)] \\
%         &=-\E_{z\sim Q(z|a, q, \gG)}Q(z|a, q, \gG)\log P_\theta(z|q) + \text{CONST}\\
%         &\geq - \sum_{z\in Q(z|a, q, \gG)}\log P_\theta(z|q).
%     \end{aligned}
% \end{equation}

% For the retrieval-then-reasoning module, we follow the FiD model \citep{izacard2021leveraging}, which allows reasoning on multiple retrieved reasoning paths, which is formulated as
% \begin{equation}
%     P_\theta(a|q,\gZ,\gG) = \prod_{z\in\gZ}P_\theta(a|q,z,\gG).
% \end{equation}

% By approximating the expectation with K sampled plans $\gZ_{K}$, the final 
% objective function can be written as
% \begin{equation}
%     \label{eq:final_obj}
%     \gL = \log P_\theta(a|\gZ_K,q,\gG) + \sum_{z\in Q(z|a, q, \gG)}\log P_\theta(z|q).
% \end{equation}
% From \eqref{eq:final_obj}, we can see that we adopt the same LLMs for both planning and reasoning, which are jointly trained on two instruction-tuning tasks. In this way, we can better distill knowledge from KGs to improve the reasoning ability of LLMs.


==> sections/conclusion.tex <==
\section{Conclusion}
In this paper, we propose a novel method called reasoning on graphs (\ourmethod) that synergizes LLMs with KGs to conduct faithful and interpretable reasoning. To \RE{alleviate} the issues of hallucinations and lack of knowledge, we present a planning-retrieval-reasoning framework, which allows LLMs to access the latest knowledge while reasoning based on faithful plans on graphs. \ourmethod not only enhances the reasoning capability of LLMs by distilling knowledge from KGs through training but also enables seamless integration with any LLMs during inference. Extensive experiments on two benchmark KGQA datasets demonstrate the superiority of \ourmethod in reasoning ability and interpretability.

==> sections/experiment.tex <==
\section{Experiment}
In our experiments, we aim to answer the following research questions:
\textbf{RQ1:} Can \ourmethod achieve state-of-the-art performance on the KGQA tasks?
\textbf{RQ2:} Can the planning module of \ourmethod be integrated with other LLMs to improve their performance?
% \textbf{RQ3:} Can \ourmethod be finetuned and effectively transferred to other knowledge graphs?
\textbf{RQ3:} Can \ourmethod conduct faithful reasoning and generate interpretable reasoning results?


\subsection{Experiment Settings}
% \input{tables/datasets.tex}
\noindent\textbf{Datasets.} 
We evaluate the reasoning ability of \ourmethod on two benchmark KGQA datasets: WebQuestionSP (WebQSP) \citep{yih2016value} and Complex WebQuestions (CWQ) \citep{talmor2018web}, which contain up to 4-hop questions. Freebase \citep{bollacker2008freebase} is the background knowledge graph for both datasets, which contains around 88 million entities, 20 thousand relations, and 126 million triples. The details of the datasets are described in \Cref{app:dataset}. 


\noindent\textbf{Baselines.} We compare \ourmethod with 21 baselines grouping into 5 categories: 1) Embedding-based methods, 2) Retrieval-augmented methods, 3) Semantic parsing methods, 4) LLMs, and 5) LLMs+KGs methods. The details of each baseline are described in \Cref{app:baselines}.

\noindent\textbf{Evaluation Metrics.} Following previous works, we use Hits@1 and F1 as the evaluation metrics. Hits@1 measures the proportion of questions whose top-1 predicted answer is correct. Since a question may correspond to multiple answers, F1 considers the coverage of all answers, which balances the precision and recall of the predicted answers.

\noindent\textbf{Implementations.} For \ourmethod, we use LLaMA2-Chat-7B \citep{touvron2023llama} as the LLM backbone, which is instruction finetuned on the training split of WebQSP and CWQ as well as Freebase for 3 epochs. We generate the top-3 relation paths using beam-search for each question. Since UniKGQA \citep{jiang2022unikgqa} and DECAF \citep{yu2022decaf} are state-of-the-art methods, we directly refer their results and those of the other baselines reported in their papers for comparisons. For LLMs, we use zero-shot prompting to conduct KGQA. The detailed settings are described in \Cref{app:settings}.

\input{tables/kgqa.tex}

\subsection{RQ1: KGQA Performance Comparison}
\noindent\textbf{Main Results.} In this section, we compare \ourmethod with other baselines on KGQA tasks. The results are shown in \Cref{tab:kgqa}. Our method achieves the best performance on both datasets across most metrics. Specifically, compared to the SOTA method DECAF~\citep{yu2022decaf} on WebQSP, our method improves Hits@1 by 4.4\%. On the CWQ dataset, which is more challenging due to multi-hop questions, our method improves both Hits@1 and F1 by 22.3\% and 14.4\% against the SOTA model UniKGQA~\citep{jiang2022unikgqa}. These results demonstrate the superior reasoning ability of our method in KGQA.

Among other methods, retrieval-augmented approaches outperform conventional embedding-based methods by retrieving relevant subgraphs from KGs, which reduces reasoning complexity. Furthermore, SR+NSM and SR+NSM+E2E adopt relation paths-based retrieval which achieves better performance, highlighting the importance of relation paths.
%
Semantic parsing methods perform better than retrieval methods on WebQSP but worse on CWQ due to the complexity of generating logical queries for complex questions in CWQ. Although LLMs-based methods achieve comparable performance, they are limited by hallucinations and lack of knowledge as shown in \Cref{sec:cases}. The LLMs+KGs methods achieve the second-best performance, which demonstrates the effectiveness of unifying KGs and LLMs for reasoning.

\textbf{Ablation Study.} We conduct an ablation study to analyze the effectiveness of the \emph{planning module} and \emph{reasoning module} in our method (\ourmethod). We compare four variants: 1) \emph{w/o planning}, where we remove the planning module and perform reasoning without retrieved reasoning paths; 2) \emph{w/o reasoning}, where we remove the reasoning module and use all answers from retrieved reasoning paths as results; 3) \emph{w/ random plans}, where we randomly retrieve reasoning paths from KGs and feed them into the reasoning module; 4) \emph{w/ vote reasoning}, where we adopt the majority voting to select top-5 answers from retrieved reasoning paths. The results are shown in \Cref{tab:ablation}.

\input{tables/ablation.tex}


From the results, it is evident that without a planning module, our method degenerates to conventional LLMs that solely rely on questions as input, suffering from the lack of knowledge issue. Although removing the reasoning module leads to high recall due to an increased number of answers, precision drops significantly because of noise in retrieved paths. This demonstrates the effectiveness of the reasoning module in identifying important reasoning paths and filtering out noise. Furthermore, using random plans achieves worse performance than removing the planning module, highlighting the importance of a planning module who generates faithful reasoning plans. Using a simple majority vote reasoning can improve the results which also demonstrate the necessity of reasoning module.

\begin{figure}[]
    \begin{center}
    %\framebox[4.0in]{$\;$}
    \includegraphics[width=0.7\columnwidth,trim=0 2mm 0 0,clip]{images/k-beam.pdf}
    \end{center}
    \vspace{-4mm}
    \caption{Faithfulness of top-$K$ generated relation paths. \emph{Green bars} denote the average number of retrieved reasoning paths, \emph{solid lines} denote the answer coverage of the retrieved paths, and \emph{dashed line} denote the answer coverage of the reasoning module based on the retrieved reasoning paths.}
    \label{fig:k-beam}
    \vspace{-7mm}
\end{figure}

\subsection{RQ2: Plug-and-Play \ourmethod Planning Module}
\input{tables/plug-and-play.tex}
In this section, we evaluate the effectiveness of integrating the planning module of \ourmethod with different LLMs during inference to improve their performance. Specifically, we first adopt the planning module of \ourmethod to generate relation paths and feed the retrieved reasoning paths as context into different LLMs for reasoning. The results are presented in \Cref{tab:plug-and-play}. To account for the fact that it is difficult to extract the number of answers from LLM's output. We only report the Hits@1 and Recall metrics. 

From the results, we can notice that the performance of all LLMs is substantially improved by integrating the planning module of \ourmethod. Specifically, the Hits@1 of ChatGPT, Alpaca, LLaMA2, and Flan-T5 are improved by 8.5\%, 15.3\%, and 119.3\%, respectively. This demonstrates that the planning module of \ourmethod can be seamlessly integrated with other LLMs to improve their performance without retraining.

% \input{tables/transfer.tex}

% \subsection{RQ3: Transferability to Other KGs}
% We also evaluate the transferability of \ourmethod to other KGs. We select the MetaQA-3hop dataset \citep{zhang2018variational} which is based on Wiki-Movies KGs\footnote{\url{https://research.fb.com/downloads/babi.}}. We select 1000 samples from the training split and utilize two training strategies to finetune \ourmethod: 1) \emph{training from scratch}, where we directly optimize \ourmethod with 1000 samples; 2) \emph{transfer from Freebase}, where we conduct a further finetuning based on \ourmethod trained for Freebase. The results are shown in \Cref{tab:transfer}. From results, we can see that transfer from Freebase achieves better performance than training from scratch, which demonstrates the transferability of \ourmethod to other KGs.

\subsection{RQ3: Faithful reasoning and interpretable results}\label{sec:cases}
\noindent\textbf{Quantitative Results.} To evaluate the faithfulness of the relation paths, we illustrate the quantitative results in \Cref{fig:k-beam}. In experiments, we sweep the number of top-$K$ relation paths generated by \ourmethod. From results, we can see that the number of retrieved reasoning paths increases with $K$, which also leads to more answers to be covered (recall). This demonstrates the faithfulness of the relation paths by retrieving the answers. However, more retrieved reasoning paths also lead to more noise and retrieval time (shown in \Cref{app:retrieval_cost}), which decreases the precision and makes little contribution to the final results (reasoning-f1). Therefore, we set $K=3$ in experiments.


\input{tables/case_study.tex}

\noindent\textbf{Case studies.} We also illustrate two case studies in \Cref{tab:case1} and \Cref{tab:case2}. In \Cref{tab:case1}, we can find that ChatGPT+CoT suffers from the lack of knowledge issue and cannot answer the question. On the contrary, \ourmethod can generate faithful relation paths and retrieve valid reasoning paths from KGs for reasoning. Besides, \ourmethod can provide interpretable explanations based on the reasoning paths. In \Cref{tab:case2}, we can see that ChatGPT+CoT suffers from hallucinations and generates incorrect answers. In contrast, although the retrieved reasoning paths contain noises, the reasoning module can identify the correct reasoning paths and conduct faithful reasoning. These results demonstrate the effectiveness of \ourmethod in conducting faithful reasoning and generating interpretable results. More cases can be found in \Cref{app:case_rel,app:case_inter}.



==> sections/introduction.tex <==
\section{Introduction}
Large language models (LLMs) have shown great performance in many NLP tasks \citep{brown2020language,bang2023multitask}. What's especially striking is their ability to handle complex tasks through reasoning \citep{wei2022chain,huang2022towards}. To further unleash LLMs' reasoning ability, the plan-and-solve paradigm \citep{wang2023plan} has been proposed, in which LLMs are prompted to generate a plan and execute each reasoning step. In this way, LLMs decompose complex reasoning tasks into a series of sub-tasks and solve them step by step \citep{khot2022decomposed}. 

Despite their success, LLMs are still limited by the lack of knowledge and prone to hallucinations during reasoning, which can lead to errors in reasoning processes \citep{hong2023faithful,wang2023knowledge}. For example, as shown in \Cref{fig:intro}, LLMs do not have the latest knowledge and hallucinate an incorrect reasoning step: ``has a daughter''. These issues largely diminish the performance and trustworthiness of LLMs in high-stakes scenarios, such as legal judgment and medical diagnosis. 

To tackle the issues, knowledge graphs (KGs) have been incorporated to improve the reasoning ability of LLMs \citep{pan2023unifying,luo2023chatrule}. KGs capture abundant factual knowledge in a structured format, which provides a faithful knowledge source for reasoning. As a typical reasoning task, knowledge graph question answering (KGQA) aims to obtain answers based on knowledge from KGs \citep{sun2019pullnet}. Previous works that jointly use KGs and LLMs for KGQA reasoning can be broadly divided into two categories: 1) semantic parsing methods \citep{lan2020query,ye2022rng}, which use LLMs to convert questions into logical queries that are executed on KGs to obtain answers; and 2) retrieval-augmented methods \citep{li2023graph,jiang2023reasoninglm}, which retrieve triples from KGs as knowledge context and uses LLMs to obtain the final answers. 

Although semantic parsing methods can generate more accurate and interpretable results by leveraging reasoning on KGs, the generated logical queries can often be non-executable and yield no answers, due to syntax and semantic limitations \citep{yu2022decaf}. Retrieval-augmented methods are more flexible and exploit the ability of LLMs for reasoning. However, they only treat KGs as factual knowledge bases and overlook the importance of their structural information for reasoning \citep{jiang2022unikgqa}. For instance, as shown in \Cref{fig:intro}, a \emph{relation path}, which is a sequence of relations, ``\texttt{child\_of}$\to$\texttt{has\_son}'' can be used to obtain answers to the question ``Who is the brother of Justin Bieber?''.  Therefore, it is essential to enable LLMs to directly reason on KGs to achieve faithful and interpretable reasoning.

In this paper, we propose a novel method called reasoning on graphs (\ourmethod) that synergizes LLMs with KGs to conduct faithful and interpretable reasoning. To \RE{alleviate} the issues of hallucinations and lack of knowledge, we present a \emph{planning-retrieval-reasoning} framework, where \ourmethod first generates relation paths grounded by KGs as faithful plans via the \emph{planning module}. These plans are then used to retrieve valid reasoning paths from KGs to conduct faithful reasoning by the \emph{retrieval-reasoning module}. In this way, we not only retrieve the latest knowledge from KGs but also consider the guidance of KG structure for reasoning and explanations. Moreover, the planning module of \ourmethod can be plug-and-play with different LLMs during inference to improve their performance.
%
Based on this framework, \ourmethod is optimized by two tasks: 1) \emph{planning optimization}, where we distill knowledge from KGs into LLMs to generate faithful relation paths as plans; and 2) \emph{retrieval-reasoning optimization}, where we enable LLMs to conduct faithful reasoning based on retrieved paths and generate interpretable results. We conduct extensive experiments on two benchmark KGQA datasets, and the results demonstrate that \ourmethod achieves state-of-the-art performance on KG reasoning tasks and generates faithful and interpretable reasoning results.
\begin{figure}[]
    \begin{center}
    %\framebox[4.0in]{$\;$}
    \includegraphics[width=.8\columnwidth,trim=0 0.3cm 0 0,clip]{images/intro.pdf}
    \end{center}
    \vspace{-4mm}
    \caption{The issues of lack of knowledge and hallucination in LLMs reasoning and how they can be addressed by triples and relation paths from KGs.}
    \label{fig:intro}
    \vspace{-5mm}
\end{figure}

==> sections/package.tex <==
\usepackage{xspace}
\usepackage{soul}
\usepackage{url}
% \usepackage[hidelinks]{hyperref}
% \usepackage[utf8]{inputenc}
% \usepackage[small]{caption}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{multirow}
\usepackage{amsthm}
\usepackage{booktabs}
% \usepackage{algorithm}
% \usepackage{algorithmic}
\usepackage{epstopdf}
\usepackage{xcolor}
\usepackage[labelformat=simple]{subcaption}
\usepackage{caption}
\usepackage{bbm}
\usepackage{dsfont}
\usepackage[ruled,linesnumbered]{algorithm2e}
%\usepackage{balance}  % for  \balance command ON LAST PAGE  (only there!)
\usepackage{setspace}
\usepackage{braket}
\usepackage{tablefootnote}
\usepackage{subcaption}
\usepackage[normalem]{ulem}
\usepackage{cleveref}
\usepackage{makecell}
\usepackage{wrapfig}
\useunder{\uline}{\ul}{}
\theoremstyle{definition}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{myDef}{Definition}[section]
\newtheorem{example}{Example}
\usepackage{tcolorbox}
% \tcbuselibrary{skins}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
\newcommand{\ourmethod}{\texttt{RoG}\xspace}
\graphicspath{{images/}}

\newcommand{\LH}[1]{\textcolor{purple}{\small\textbf{[LH]} #1 $\triangleleft$}}
\newcommand{\SP}[1]{\textcolor{orange}{\small\textbf{[SP]} #1 $\triangleleft$}}
\newcommand{\todo}[1]{{\color{red}{ [To-do: #1]}}}
\newcommand{\delete}[1]{{\color{violet}{ [DELETE: #1]}}}
\newcommand{\hlt}{\textcolor{blue}}
\newcommand{\yf}[1]{\textcolor{brown}{\small\textbf{[YF]} #1 $\triangleleft$}}
\newcommand{\RE}{\textcolor{black}}

==> sections/preliminary.tex <==
\section{Preliminary}

\noindent\textbf{Knowledge Graphs (KGs)} contain abundant factual knowledge in the form of a set of triples: $\gG=\{(e,r,e')|e,e'\in\gE,r\in\gR\}$, where $\gE$ and $\gR$ denote the set of entities and relations, respectively.

\noindent\textbf{Relation Paths} are a sequence of relations: $z=\{r_1,r_2,\dots,r_l\}$, where $r_i\in\gR$ denotes the $i$-th relation in the path and $l$ denotes the length of the path.

\noindent\textbf{Reasoning Paths} are the instances of a relation path $z$ in KGs: $w_z=e_0\xrightarrow{r_1}e_1\xrightarrow{r_2}\ldots\xrightarrow{r_l}e_{l}$, where $e_i\in\gE$ denotes the $i$-th entity and $r_i$ denotes the $i$-th relation in the relation path $z$.
%Relation paths expressing the semantic relations between entities have been used in many KG reasoning tasks \citep{das2018go,cui2023path}. 
\begin{example}
        Given a relation path: $z=\texttt{marry\_to}\to\texttt{father\_of}$, a reasoning path instance could be: $w_z=\text{Alice}\xrightarrow{\texttt{marry\_to}}\text{Bob}\xrightarrow{\texttt{father\_of}}\text{Charlie}$, which denotes ``Alice'' is married to ``Bob'' and ``Bob'' is the father of ``Charlie''.
\end{example}

\noindent\textbf{Knowledge Graph Question Answering (KGQA)} is a typical reasoning task based on KGs. Given a natural language question $q$ and a KG $\gG$, the task aims to design a function $f$ to predict answers $a\in\gA_q$ based on knowledge from $\gG$, i.e., $a=f(q,\gG)$. Following previous works \citep{sun2019pullnet,jiang2022unikgqa}, we assume the entities $e_q\in\gT_q$ mentioned in $q$ and answers $a\in\gA_q$ are labeled and linked to the corresponding entities in $\gG$, i.e., $\gT_q,\gA_q\subseteq\gE$.

==> sections/relatedworks.tex <==
\section{Related Work}


\vspace{-2mm}
\noindent\textbf{LLM Reasoning Prompt.}
Many studies have been proposed to harness the reasoning ability of LLMs to handle complex tasks through prompting \citep{wei2022chain,wang2022self,yao2023tree,besta2023graph}. Plan-and-solve \citep{wang2023plan} prompts LLMs to generate a plan and conduct reasoning based on it. DecomP \citep{he2021improving} prompts LLMs to decompose the reasoning task into a series of sub-tasks and solve them step by step.
However, the problem of hallucinations and lack of knowledge affect the faithfulness of LLMs' reasoning. ReACT \citep{yao2022react} treats LLMs as agents, which interact with the environment to get the latest knowledge for reasoning. To explore faithful reasoning, FAME \citep{hong2023faithful} introduces the Monte-Carlo planning to generate faithful reasoning steps. RR \citep{he2022rethinking} and KD-CoT \cite{wang2023knowledge} further retrieve relevant knowledge from KGs to produce faithful reasoning plans for LLMs. 

\noindent\textbf{Knowledge Graph Question Answering (KGQA).}
Conventional \emph{embedding-based methods} represent the entities and relations in embedding space and design special model architectures (e.g., Key-Value memory networks, sequential models, and graph neural networks) to reason answers \citep{miller2016key,he2021improving,yasunaga2021qa}. To integrate LLMs for KGQA, \emph{retrieval-augmented methods} aim to retrieve the relative facts from the KGs to improve the reasoning performance \citep{li2023graph,karpukhin2020dense}. Recently, UniKGQA \citep{jiang2022unikgqa} which unifies the graph retrieval and reasoning process into a single model with LLMs, achieves STOA performance. \emph{Semantic parsing methods} convert the question into a structural query (e.g., SPARQL) by LLMs, which can be executed by a query engine to reason the answers on KGs \citep{sun2020sparqa,lan2020query}. However, these methods heavily rely on the quality of generated queries. If the query is not executable, no answers will be generated. DECAF \citep{yu2022decaf} combines semantic parsing and LLMs reasoning to jointly generate answers, which also reach salient performance on KGQA tasks.


==> sections/statement.tex <==
\section*{Ethics Statement}
Our work is solely dedicated to tackling scientific problems and does not involve any human subjects, animals, or environmentally sensitive materials. Consequently, we do not anticipate any potential ethical risks or conflicts of interest in our study. Our research strives to adhere to the highest standards of scientific integrity and ethical conduct throughout the entire process, guaranteeing the validity and reliability of our findings.

\section*{Reproducibility Statement}
Our model has been meticulously formalized within the main body of the text to ensure clarity and facilitate comprehensive understanding. Additionally, we provide detailed discussions of implementation in \Cref{app:dataset,app:baselines,app:settings}, encompassing dataset information, baselines, experimental settings, and model configurations. The code and pre-trained model weights have been publicized.

==> tables/ablation.tex <==
% \begin{table}[]
\begin{wraptable}{r}{.6\columnwidth}
    \centering
    \vspace{-5mm}
    \caption{Ablation studies of \ourmethod.}
      \vspace{-3mm}
    \label{tab:ablation}
    \resizebox{.6\columnwidth}{!}{%
    \begin{tabular}{@{}l|ccc|ccc@{}}
        \toprule
        \multirow{2}{*}{Method}    & \multicolumn{3}{c|}{WebQSP} & \multicolumn{3}{c}{CWQ}                                                                     \\ \cmidrule(l){2-7}
                                   & Precision                   & Recall                  & F1             & Precision      & Recall         & F1             \\ \midrule
        \ourmethod                 & \textbf{74.77}              & 75.84                   & \textbf{70.81} & \textbf{57.69} & 58.19          & \textbf{56.17} \\ \midrule
        \ourmethod w/o planning    & 57.26                       & 50.16                   & 49.69          & 35.35          & 34.77          & 33.76          \\
        \ourmethod w/o reasoning   & 46.90                       & \textbf{79.85}          & 49.56         & 18.88         & \textbf{67.89} & 22.26          \\\midrule
        \ourmethod w/ random plans & 38.66                       & 38.31                   & 35.24          & 38.99          & 39.29          & 37.64          \\ 
        \ourmethod w/ vote reasoning & 54.80	& 60.44	& 47.96	& 22.92	& 47.98	& 26.52 \\ 
        \bottomrule
    \end{tabular}%
    }
    \vspace{-4mm}
\end{wraptable} 
% \end{table}

==> tables/case_int.tex <==
\begin{table}[]
    \centering
    \caption{Examples of faithful and interpretable reasoning of \ourmethod.}
    \vspace{-3mm}
    \label{tab:case_int}
    \resizebox{1\columnwidth}{!}{%
    \begin{tabular}{@{}c|p{5in}@{}}
        \toprule
        Question             & Lou Seal is the mascot for the team that last won the World Series when?                                                                                                                                                                                                                                                                                         \\ \midrule
        Answer               & 2014                                                                                                                                                                                                                                                                                                                                                 \\ \midrule
        Reasoning Paths      & Lou Seal $\to$ sports.mascot.team $\to$ San Francisco Giants $\to$ sports.sports\_championship\_event.champion $\to$ 2014 World Series                                                                                                                                                                                        \\
        \midrule
        \ourmethod & \begin{tabular}[c]{@{}p{5in}@{}}Based on the provided reasoning paths, we can determine when the team for which Lou Seal is the mascot last won the World Series:\\\\

            1. Lou Seal is associated with the San Francisco Giants.\\
            2. The San Francisco Giants are associated with winning the 2014 World Series.\\\\
            
            Therefore, the San Francisco Giants, the team for which Lou Seal is the mascot, last won the World Series in 2014.\end{tabular}                                                                                                                                                                                                                                                                                                                                            \\ \bottomrule
            \toprule
            Question             & what is my timezone in louisiana?                                                                                                                                                                                                                                                                                         \\ \midrule
            Answer               & Central Time Zone                                                                                                                                                                                                                                                                                                                                                 \\ \midrule
            Reasoning Paths      & \begin{tabular}[c]{@{}p{5in}@{}} Louisiana $\to$ location.location.partially\_containedby $\to$ Tangipahoa River $\to$ geography.river.origin $\to$ Osyka $\to$ location.location.time\_zones $\to$ Central Time Zone \\\\
                Louisiana $\to$ location.location.containedby $\to$ Alexandria $\to$ location.location.containedby $\to$ United States of America $\to$ location.location.time\_zones $\to$ Central Time Zone 
            \end{tabular}\\
        \midrule
            \ourmethod & \begin{tabular}[c]{@{}p{5in}@{}}Based on the reasoning paths provided, it can be determined that Louisiana is in the Central Time Zone. \\\\

                Here's the explanation: \\\\
                
                1. The first reasoning path tells us that Louisiana is partially contained by the Tangipahoa River, which is a geographical feature. However, it doesn't directly mention the time zone. \\\\
                
                2. The second reasoning path establishes that Louisiana is contained by Alexandria, which is in turn contained by the United States of America. The United States of America is in the Central Time Zone. \\\\
                
                Therefore, based on these reasoning paths, the time zone in Louisiana is the Central Time Zone.\end{tabular}                                                                                                                                                                                                                                                                                                                                            \\ \bottomrule
                \toprule
                Question             & Which child of Walt Disney died from lung cancer?                                                                                                                                                                                                                                                                                         \\ \midrule
                Answer               & Sharon Mae Disney                                                                                                                                                                                                                                                                                                                             \\ \midrule
                Reasoning Paths      & \begin{tabular}[c]{@{}p{5in}@{}} Lung cancer $\to$ people.deceased\_person.cause\_of\_death $\to$ Sharon Mae Disney\\\\
                    Lung cancer $\to$ people.deceased\_person.cause\_of\_death $\to$ Walt Disney \\\\
                    Walt Disney $\to$ people.deceased\_person.cause\_of\_death $\to$ Lung cancer \\\\
                    Walt Disney $\to$ people.person.children $\to$ Diane Disney Miller \\\\
                    Walt Disney $\to$ people.cause\_of\_death.people $\to$ Circulatory collapse \\\\
                    Walt Disney $\to$ people.person.parents $\to$ Flora Call Disney \\\\
                    Walt Disney $\to$ people.person.parents $\to$ Elias Disney \\\\
                    Walt Disney $\to$ people.person.parents $\to$ Sharon Mae Disney
                \end{tabular}\\
            \midrule
                \ourmethod & \begin{tabular}[c]{@{}p{5in}@{}}Based on the reasoning paths provided, it appears that Sharon Mae Disney is the child of Walt Disney who died from lung cancer.\\\\ 
                    
                The reasoning path "Walt Disney $\to$ people.deceased\_person.cause\_of\_death $\to$ Lung cancer" directly connects Walt Disney to lung cancer as a cause of death, and since Sharon Mae Disney is also linked to lung cancer as a cause of death through the path "Lung cancer $\to$ people.deceased\_person.cause\_of\_death $\to$ Sharon Mae Disney," it can be concluded that Sharon Mae Disney is the child of Walt Disney who died from lung cancer.\end{tabular}                                                                                                                                                                                                                                                                                                                                            \\ \bottomrule
    \end{tabular}}
\end{table}

==> tables/case_rel.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[h]
    \centering
    \caption{Examples of the generated relation paths.}
    \label{tab:case_rel}
    \resizebox{.97\columnwidth}{!}{%
        \begin{tabular}{@{}p{2.5in}|l@{}}
            \toprule
            Question                                                                                                      &
            Top-3 Relation Paths                                                                                            \\\midrule
            what does jamaican people speak?                                                                               &
            \begin{tabular}[c]{@{}l@{}}$z_1:$   location.country.languages\_spoken\\      $z_2:$ language.human\_language.countries\_spoken\_in\\      $z_3:$ location.country.official\_language\end{tabular}                                                                                       \\\midrule
            where is jamarcus russell from?                                                                                &
            \begin{tabular}[c]{@{}l@{}}$z_1:$   location.location.people\_born\_here\\      $z_2:$ people.person.place\_of\_birth\\      $z_3:$ sports.sports\_league\_draft\_pick.player $\to$   sports.sports\_league\_draft\_pick.location\end{tabular}                                                                                       \\ \midrule
            where did edgar allan poe died?                                                                                &
            \begin{tabular}[c]{@{}l@{}}$z_1:$   people.deceased\_person.place\_of\_death\\      $z_2:$ people.cause\_of\_death.people\\      $z_3:$ people.person.place\_of\_birth\end{tabular}                                                                                       \\ \midrule
            what highschool did harper lee go to?                                                                          &
            \begin{tabular}[c]{@{}l@{}}$z_1:$ people.person.education   $\to$ education.educational\_institution.students\_graduates\\      $z_2:$ education.education.student $\to$   education.educational\_institution.students\_graduates\\      $z_3:$ people.person.education $\to$ education.education.institutio\end{tabular}                                                                                       \\ \midrule
            what are the songs that justin bieber   wrote?                                                                 &
            \begin{tabular}[c]{@{}l@{}}$z_1:$   music.recording.artist\\      $z_2:$ music.composition.composer\\      $z_3:$ music.composer.compositions\end{tabular}                                                                                       \\ \midrule
            what are the religions practiced in   indonesia?                                                               &
            \begin{tabular}[c]{@{}l@{}}$z_1:$ people.person.nationality   $\to$ people.person.religion\\      $z_2:$ location.statistical\_region.religions $\to$   location.religion\_percentage.religion\\      $z_3:$ location.country.languages\_spoken $\to$ religion.religion.languages\end{tabular}                                                                                       \\ \midrule
            Lou Seal is the mascot for the team that   last won the World Series when?                                    &
            \begin{tabular}[c]{@{}l@{}}$z_1:$ sports.mascot.team $\to$   sports.sports\_championship\_event.champion\\      $z_2:$ sports.mascot.team $\to$ sports.sports\_team.championships\\      $z_3:$ sports.sports\_championship\_event.championship\end{tabular}                                                                                       \\ \midrule
            % What country in the Caribbean contains Saint Michael Parish? & \begin{tabular}[c]{@{}l@{}}$z_1:$  location.administrative\_division.first\_level\_division\_of\\      $z_2:$ location.location.containedby\\      $z_3:$ location.location.contains\end{tabular} \\ \midrule
            What type of government is used in the   country with Northern District?                                      &
            \begin{tabular}[c]{@{}l@{}}$z_1:$   location.administrative\_division.first\_level\_division\_of $\to$   government.form\_of\_government.countries\\      $z_2:$ location.administrative\_division.first\_level\_division\_of $\to$   location.country.form\_of\_government\\      $z_3:$ administrative\_division.first\_level\_division\_of $\to$   government.form\_of\_government.countries\end{tabular}                                                                                       \\ \midrule
            The people from the country that contains   Nord-Ouest Department speak what languages today?                 &
            \begin{tabular}[c]{@{}l@{}}$z_1:$   location.administrative\_division.first\_level\_division\_of $\to$   language.human\_language.countries\_spoken\_in\\      $z_2:$ location.administrative\_division.first\_level\_division\_of $\to$   location.country.languages\_spoken\\      $z_3:$ base.aareas.schema.administrative\_area.administrative\_parent $\to$   location.country.languages\_spoken\end{tabular}                                                                                       \\ \midrule
            What stadium does the team with mascot   named Hank play at?                                                  &
            \begin{tabular}[c]{@{}l@{}}$z_1:$ sports.mascot.team $\to$   sports.sports\_facility.teams\\      $z_2:$ sports.sports\_team.team\_mascot $\to$   sports.sports\_facility.teams\\      $z_3:$ sports.mascot.team $\to$ sports.sports\_team.arena\_stadium\end{tabular}                                                                                      \\ \midrule
            Which popular sports team in Spain, that   won the 2014 Eurocup Finals championship?                          &
            \begin{tabular}[c]{@{}l@{}}$z_1:$   sports.sports\_team.championships $\to$   sports.sports\_team\_location.teams\\      $z_2:$ sports.sports\_team.location $\to$   sports.sports\_team\_location.teams\\      $z_2:$ sports.sports\_team.location $\to$   sports.sports\_team\_location.teams\\      $z_3:$ sports.sports\_team\_location.teams\end{tabular}                                                                                      \\ \midrule
            What educational institution with the   mascot named Washington University Bear did Tennessee Williams go to? &
            \begin{tabular}[c]{@{}l@{}}$z_1:$   education.educational\_institution.mascot\\      $z_2:$ people.person.nationality $\to$ location.location.containedby\\      $z_3:$ education.education.student $\to$ education.education.institution\end{tabular}\\ \midrule
            Who is the current head coach of the NFL squad owned by the Rooney family? & \begin{tabular}[c]{@{}l@{}}$z_1:$   sports.professional\_sports\_team.owner\_s $\to$ american\_football.football\_coach.current\_team\_head\_coached\\      $z_2:$ sports.professional\_sports\_team.owner\_s $\to$ american\_football.football\_team.current\_head\_coach\\      $z_3:$ american\_football.football\_coach.current\_team\_head\_coached \end{tabular}\\\midrule

            What is the home field of the sports team whose mascot is named Fredbird? & \begin{tabular}[c]{@{}l@{}}$z_1:$   sports.mascot.team $\to$ sports.sports\_facility.teams\\      $z_2:$ sports.sports\_team.team\_mascot $\to$ sports.sports\_facility.teams\\      $z_3:$ sports.mascot.team $\to$ sports.sports\_team.arena\_stadium \end{tabular}\\
            \bottomrule
        \end{tabular}%
    }
\end{table}

==> tables/case_study.tex <==
\begin{table}[]
    \centering
    \caption{Example of \textit{lack of knowledge} for ChatGPT-CoT and interpretable predictions of \ourmethod.}
    \vspace{-3mm}
    \label{tab:case1}
    \resizebox{.7\columnwidth}{!}{%
    \begin{tabular}{@{}c|p{5in}@{}}
        \toprule
        Question             & What type of government is used in the country with Northern District?                                                                                                                                                                                                                                                                                               \\ \midrule
        Answer               & Parliamentary system                                                                                                                                                                                                                                                                                                                                                 \\ \midrule
        ChatGPT + CoT        & To determine what type of government is used in a country with a Northern District, \textcolor{red}{we need more specific information}. The term "Northern District" does not specify the name of any particular country or provide enough context to identify its government type. \textcolor{red}{Could you please provide additional details or clarify the specific country you are referring to?} \\ \midrule
        Reasoning Paths      & Northern District $\to$ location.administrative\_division.first\_level\_division\_of $\to$ Israel $\to$ government.form\_of\_government.countries $\to$ \textbf{Parliamentary system}                                                                                                                                                                                         \\
        \midrule
        \ourmethod & \begin{tabular}[c]{@{}p{5in}@{}}The type of government used in the country with the Northern District is a \textbf{Parliamentary system}.\\\\  Explanations:\\ \\ 1. Northern District $\to$ location.administrative\_division.first\_level\_division\_of $\to$ Israel: \\ The Northern District is a part of Israel.\\ 2. Israel $\to$ government.form\_of\_government.countries $\to$ Parliamentary system: Israel has a Parliamentary system of government.\\ \\ So, by following the reasoning paths provided, we can conclude that the country with the Northern District, which is Israel, uses a Parliamentary system of government.\end{tabular}                                                                                                                                                                                                                                                                                                                                            \\ \bottomrule
    \end{tabular}}
    \vspace{-3mm}
\end{table}


\begin{table}[]
    \centering
    \caption{Example of the \textit{hallucination} of ChatGPT-CoT and faithful reasoning of \ourmethod.}
    \vspace{-3mm}
    \label{tab:case2}
    \resizebox{.7\columnwidth}{!}{%
    \begin{tabular}{@{}c|p{5in}@{}}
        \toprule
        Question             & Where is the home stadium of the team who won the 1946 World Series championship?
        \\ \midrule
        Answer               & Busch Stadium                                                                                                                                                                                                                                                                                                                                                 \\ \midrule
        ChatGPT + CoT        & \begin{tabular}[c]{@{}p{5in}@{}}Step 1: Identify the team that won the 1946 World Series championship.
            The team that won the 1946 World Series championship was the St. Louis Cardinals. \\\\
            
            Step 2: Determine the home stadium of the St. Louis Cardinals during that time. The St. Louis Cardinals' home stadium during the 1946 season was  \textcolor{red}{Sportsman's Park}. \\\\
            
            Therefore, the possible answer to the question "Where is the home stadium of the team who won the 1946 World Series championship?" is:
            -  \textcolor{red}{Sportsman's Park}.\end{tabular}
             \\ \midrule
        Reasoning Paths      & \begin{tabular}[c]{@{}p{5in}@{}} 1946 World Series $\to$ sports.sports\_team.championships $\to$ St. Louis Cardinals $\to$ sports.sports\_team.arena\_stadium $\to$ \textbf{Busch Stadium}\\
            1946 World Series $\to$ sports.sports\_team.championships $\to$ St. Louis Cardinals $\to$ sports.sports\_team.arena\_stadium $\to$ \textcolor{red}{Roger Dean Stadium}\end{tabular}\\
        \midrule
        \ourmethod & \begin{tabular}[c]{@{}p{5in}@{}}Based on the reasoning paths provided, the home stadium of the team who won the 1946 World Series championship is \textbf{Busch Stadium}. This conclusion is based on the following path:\\\\

            \textbf{1. 1946 World Series $\to$ sports.sports\_team.championships $\to$ St. Louis Cardinals $\to$ sports.sports\_team.arena\_stadium $\to$ Busch Stadium} \\\\
            
            The reasoning path leads us to the St. Louis Cardinals as the team that won the 1946 World Series, and Busch Stadium is the stadium associated with the St. Louis Cardinals. Therefore, \textbf{Busch Stadium} is the home stadium of the team that won the 1946 World Series championship.\end{tabular}                                                                                                                                                                                                                                                                                                                                            \\ \bottomrule
    \end{tabular}}
    \vspace{-5mm}
\end{table}

==> tables/datasets.tex <==
% \begin{wraptable}{r}{.35\columnwidth}
\begin{table}[]
    \centering
    % \vspace{-3mm}
    \caption{Statistics of datasets.}
    \label{tab:dataset}
    % \resizebox{.35\columnwidth}{!}{%
    \begin{tabular}{@{}c|ccc@{}}
        \toprule
        Datasets & \#Train & \#Test & Max \#hop \\ \midrule
        WebQSP   & 2,826   & 1,628  & 2         \\
        CWQ      & 27,639  & 3,531  & 4         \\ \bottomrule
    \end{tabular}%
    % }
    % \vspace{-3mm}
% \end{wraptable} 
\end{table}

==> tables/ft_llm.tex <==
\begin{table}[]
    \centering
    \caption{Performance comparison with different finetuned LLMs (Hits@1).}
    \label{tab:ft_llm}
    \RE{
    %\resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}ccc@{}}
    \toprule
    Method                      & WebQSP         & CWQ            \\ \midrule
    Alpaca-7B (Zero Shot)      & 51.78          & 27.44          \\
    LLaMA2-Chat-7B (Zero Shot) & 64.37          & 34.60          \\
    Alpaca-7B (Finetuned)       & 74.57          & 55.98          \\
    LLaMA2-Chat-7B (Finetuned)  & 73.89          & 53.49          \\\midrule
    \ourmethod                  & \textbf{85.75} & \textbf{62.65} \\ \bottomrule
    \end{tabular}%
    }
\end{table}

==> tables/kgqa.tex <==
\begin{table}[]
    \centering
    \caption{Performance comparison with different baselines on the two KGQA datasets.}
      \vspace{-3mm}
    \label{tab:kgqa}
    \resizebox{.7\columnwidth}{!}{%
    \begin{tabular}{@{}c|llccc@{}}
        \toprule
        \multirow{2}{*}{Type}             & \multirow{2}{*}{Methods}                & \multicolumn{2}{c}{WebQSP}    & \multicolumn{2}{c}{CWQ}       \\ \cmidrule(l){3-6} 
                                          &                                         & Hits@1        & F1            & Hits@1        & F1            \\ \midrule
        \multirow{5}{*}{Embedding}        & KV-Mem \citep{miller2016key}            & 46.7          & 34.5          & 18.4          & 15.7          \\
                                          & EmbedKGQA \citep{saxena2020improving}   & 66.6          & -             & 45.9          & -             \\
                                          & NSM \citep{he2021improving}             & 68.7          & 62.8          & 47.6          & 42.4          \\
                                          & TransferNet \citep{shi2021transfernet}  & 71.4          & -             & 48.6          & -             \\
                                          & KGT5 \cite{saxena2022sequence}          & 56.1          & -             & 36.5          & -             \\ \midrule
        \multirow{4}{*}{Retrieval}        & GraftNet \citep{sun2018open}            & 66.4          & 60.4          & 36.8          & 32.7          \\
                                          & PullNet \citep{sun2019pullnet}          & 68.1          & -             & 45.9          & -             \\
                                          & SR+NSM \citep{zhang2022subgraph}        & 68.9          & 64.1          & 50.2          & 47.1          \\
                                          & SR+NSM+E2E \citep{zhang2022subgraph}    & 69.5          & 64.1          & 49.3          & 46.3          \\ \midrule
        \multirow{4}{*}{Semantic Parsing} & SPARQL \citep{sun2020sparqa}            & -             & -             & 31.6          & -             \\
                                          & QGG \citep{lan2020query}                & 73.0          & 73.8          & 36.9          & 37.4          \\
                                          & ArcaneQA \citep{gu2022arcaneqa}         & -             & 75.3          & -             & -             \\
                                          & RnG-KBQA \citep{ye2022rng}              & -             & 76.2          & -             & -             \\ \midrule
        \multirow{5}{*}{LLMs}             & Flan-T5-xl \citep{chung2022scaling}     & 31.0          & -             & 14.7          & -             \\
                                          & Alpaca-7B \citep{taoristanford}         & 51.8          & -             & 27.4          & -             \\
                                          & LLaMA2-Chat-7B \citep{touvron2023llama} & 64.4          & -             & 34.6          & -             \\
                                          & ChatGPT                                 & 66.8          & -             & 39.9          & -             \\
                                          & ChatGPT+CoT                             & 75.6          & -             & 48.9          & -             \\ \midrule
        \multirow{4}{*}{LLMs+KGs}         & KD-CoT \citep{wang2023knowledge}        & 68.6          & 52.5          & 55.7          & -             \\
                                          & UniKGQA \citep{jiang2022unikgqa}        & 77.2          & 72.2          & 51.2          & 49.1          \\
                                          & DECAF (DPR+FiD-3B) \citep{yu2022decaf}  & 82.1          & \textbf{78.8} & -             & -             \\ \cmidrule(l){2-6} 
                                          & \ourmethod             & \textbf{85.7} & 70.8          & \textbf{62.6} & \textbf{56.2} \\ \bottomrule
        \end{tabular}   
    }
    \vspace{-6mm}
\end{table}


==> tables/plug-and-play.tex <==
% \begin{table}[]
\begin{wraptable}{r}{.5\columnwidth}
    \centering
    \vspace{-4mm}
    \caption{Effects of integrating the planning module of \ourmethod with different LLMs for reasoning.}
    \vspace{-3mm}
    \label{tab:plug-and-play}
    \resizebox{.5\columnwidth}{!}{%
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        \multirow{2}{*}{Methods} & \multicolumn{2}{c}{WebQSP} & \multicolumn{2}{c}{CWQ}                                   \\ \cmidrule(l){2-5}
                                 & Hits@1                     & Recall                  & Hits@1         & Recall         \\ \midrule
        ChatGPT                  & 66.77                      & 49.27                   & 39.90          & 35.07          \\
        ChatGPT + \ourmethod Planning              & \textbf{81.51}             & \textbf{71.60}          & \textbf{52.68} & \textbf{48.51} \\ \midrule
        Alpaca-7B                & 51.78                      & 33.65                   & 27.44          & 23.62          \\
        Alpaca-7B + \ourmethod Planning              & \textbf{56.16}             & \textbf{74.20}          & \textbf{44.04} & \textbf{38.46} \\ \midrule
        LLaMA2-Chat-7B           & 64.37                      & 44.61                   & 34.60          & 29.91          \\
        LLaMA2-Chat-7B + \ourmethod Planning      & \textbf{74.20}             & \textbf{56.16}          & \textbf{56.41} & \textbf{51.99} \\ \midrule
        Flan-T5-xl                  & 30.95                      & 17.08                   & 14.69          & 12.25          \\
        Flan-T5-xl + \ourmethod Planning             & \textbf{67.87}             & \textbf{44.93}          & \textbf{37.81} & \textbf{32.57} \\ \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
\end{wraptable} 
% \end{table}

==> tables/single_dataset.tex <==

\begin{table}[]
    \centering
    \caption{Performance on WebQSP with different training data.}
    \label{tab:webqsp_only}
    %\resizebox{\columnwidth}{!}{%
    \RE{
        \begin{tabular}{@{}cccc@{}}
            \toprule
            Method     & Training Data & Hits@1 & F1   \\ \midrule
            UniKGQA    & WebQSP        & 77.2   & 72,2 \\
            \ourmethod & WebQSP        & 81.5   & 61.8 \\
            \ourmethod & WebQSP+CWQ    & 85.7   & 70.8 \\ \bottomrule
        \end{tabular}%
        %}
    }
\end{table}

\begin{table}[]
    \centering
    \caption{Performance on CWQ with different training data.}
    \label{tab:cwq_only}
    %\resizebox{\columnwidth}{!}{%
    \RE{
        \begin{tabular}{@{}cccc@{}}
            \toprule
            Method     & Training Data & Hits@1 & F1   \\ \midrule
            UniKGQA    & CWQ           & 51.2   & 49.1 \\
            \ourmethod & CWQ           & 59.1   & 52.9 \\
            \ourmethod & WebQSP+CWQ    & 62.6   & 56.2 \\ \bottomrule
        \end{tabular}%
        %}
    }
\end{table}


==> tables/transfer.tex <==
\begin{table}
    \centering
    \caption{Performance of \ourmethod on MetaQA-3hop.}
    \label{tab:transfer}
    %\resizebox{2.2in}{!}{%
    \begin{tabular}{@{}l|cc@{}}
        \toprule
        \multirow{3}{*}{Strategies}         & \multicolumn{2}{c}{MetaQA-3hop}                  \\ \cmidrule(l){2-3}
                                            & Hits@1                          & F1             \\ \midrule
        \ourmethod (train from scratch)  & 84.81                           & 41.32          \\
        \ourmethod (transfer from Freebase) & \textbf{88.98}                  & \textbf{50.68} \\ \bottomrule
    \end{tabular}
    %}
\end{table} 


\begin{table}
    \centering
    \RE{
    \caption{Training time comparison.}
    \label{tab:time}
    %\resizebox{2.2in}{!}{%
    \begin{tabular}{@{}c|cc@{}}
        \toprule
        Method & Training on Freebase & Transferring to Wiki-Movies \\
        \midrule
        \ourmethod & 38 hours & 2 hours \\
        \bottomrule
    \end{tabular}
    %}
    }
\end{table} 
